A Tiny Supervised ODL Core with Auto Data Pruning for Human Activity Recognition

In this paper, we introduce a low-cost and low-power tiny supervised on-device learning (ODL) core that can address the distributional shift of input data for human activity recognition. Although ODL for resource-limited edge devices has been studied recently, how exactly to provide the training labels to these devices at runtime remains an open-issue. To address this problem, we propose to combine an automatic data pruning with supervised ODL to reduce the number queries needed to acquire predicted labels from a nearby teacher device and thus save power consumption during model retraining. The data pruning threshold is automatically tuned, eliminating a manual threshold tuning. As a tinyML solution at a few mW for the human activity recognition, we design a supervised ODL core that supports our automatic data pruning using a 45nm CMOS process technology. We show that the required memory size for the core is smaller than the same-shaped multilayer perceptron (MLP) and the power consumption is only 3.39mW. Experiments using a human activity recognition dataset show that the proposed automatic data pruning reduces the communication volume by 55.7% and power consumption accordingly with only 0.9% accuracy loss.

==> Makefile <==
LATEX   = platex
BIBTEX  = pbibtex
DVIPS   = dvips
DVIPDF  = dvipdfmx
TARGET  = main
TEXFILE = $(TARGET).tex \
	refer.bib \
	abst.tex \
	intro.tex \
	related.tex \
	design.tex \
	eval.tex \
	conc.tex

all: $(TARGET).dvi

dvi: $(TARGET).dvi
$(TARGET).dvi: $(TEXFILE)
	#$(LATEX) $(TARGET)
	#$(BIBTEX) $(TARGET)
	$(LATEX) $(TARGET)
	$(LATEX) $(TARGET)

ps: $(TARGET).ps
$(TARGET).ps: $(TARGET).dvi
	$(DVIPS) -f $(TARGET).dvi > $(TARGET).ps

pdf: $(TARGET).pdf
$(TARGET).pdf: $(TARGET).dvi
	$(DVIPDF) $(TARGET).dvi

clean:
	rm -f $(TARGET).dvi
	rm -f $(TARGET).ps
	rm -f $(TARGET).log
	rm -f $(TARGET).pdf
	#rm -f $(TARGET).bbl
	rm -f $(TARGET).blg
	rm -f *.aux *.out *.xcp *~ 


==> related.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% related.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Related Work}\label{sec:related}

%
% Concept drift
%
Data drift is known as distributional shift of input data due to
environmental changes.
In Figure \ref{fig:cluster}, for example, the data distribution may
change depending on human subjects.
%Data drift detection methods are surveyed in \cite{Lu19}.
There are various approaches to detect the data drift.
For example, QuantTree \cite{Boracchi18} is a distribution-based
detection method that utilizes histograms or bins.
In \cite{Yamada23}, a fully-sequential detection method that considers
the distance between the centroid of trained samples and that of recent
samples is introduced.
The detection method is compared with existing ones such as
\cite{Boracchi18} 
%in terms of the accuracy, detection delay, and memory size.
in terms of the accuracy and memory size.
These methods can be used for our ODL to trigger the retraining.

%
% ODL
%
Regarding the ODL of neural networks for resource-limited edge devices,
the OS-ELM (Online Sequential Extreme Learning Machine) algorithm
\cite{Liang06} is combined with autoencoder \cite{Hinton06} for
unsupervised (or semi-supervised) anomaly detection \cite{Tsukada20}.
In this direction, ROHM announced a low-power ODL-capable chip that
consumes a few tens of mW 
for predictive failure detection in electronic devices \cite{RohmODL}.
TinyTL \cite{Cai20} is a tiny transfer learning approach for
memory-efficient ODL.
This approach freezes the weight parameters, while learning only the
bias modules to reduce memory consumption during the ODL.
TinyOL \cite{Ren21} is also a tiny transfer learning approach that can
fine-tune the last layer of pretrained neural networks.
The retrainable layer is combined with a pre-trained autoencoder and
%used for anomaly detection and multi-anomaly classification.
used for anomaly detection and classification.

In contrast with these prior works, our paper tackles the labeling
problem of ODLs while using a teacher device and wireless communication.
%
% Data pruning
%
Since our supervised ODL involves the teacher device, redundant
queries to the teacher should be eliminated.
To reduce the redundant training samples, data pruning techniques have
been studied to select a part of data (e.g., hard samples) for
training without sacrificing test accuracy.
Recently, EL2N (Error L2-Norm) score (where the error vector is the
predicted class probabilities minus one-hot encoded label) is used as
a pruning metric \cite{Paul21}.
% We should note that the teacher labels required in EL2N are
% {\it not available} at the time of label acquisition by edge devices.
% We hence introduce an efficient approach for the training data selection.
As a use case, a batch of training samples are sorted by EL2N score, and then a
fraction of samples can be pruned based on the ranking.
However, this is {\it not suited} for our online sequential training
setting, where a training sample comes one by one.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

